Analysis of Source Code Using UPPAAL

In recent years there has been a considerable effort in optimising formal methods for application to code. This has been driven by tools such as CPAChecker, DIVINE, and CBMC. At the same time tools such as Uppaal have been massively expanding the realm of more traditional model checking technologies to include strategy synthesis algorithms - an aspect becoming more and more needed as software becomes increasingly parallel. Instead of reimplementing the advances made by Uppaal in this area, we suggest in this paper to develop a bridge between the source code and the engine of Uppaal. Our approach uses the widespread intermediate language LLVM and makes recent advances of the Uppaal ecosystem readily available to analysis of source code.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{A. Paskevich, J. Proen\c{c}a (Eds.): Formal Integrated\\
Development Environment 2021 (F-IDE 2021)\\
EPTCS 338, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.338.5}{10.4204/EPTCS.338.5}}
\pdfoutput=1

